Video2GIF: Automatic Generation of Animated GIFs from Video

We introduce the novel problem of automatically generating animated GIFs from video. GIFs are short looping video with no sound, and a perfect combination between image and video that really capture our attention. GIFs tell a story, express emotion, turn events into humorous moments, and are the new wave of photojournalism. We pose the question: Can we automate the entirely manual and elaborate process of GIF creation by leveraging the plethora of user generated GIF content? We propose a Robust Deep RankNet that, given a video, generates a ranked list of its segments according to their suitability as GIF. We train our model to learn what visual content is often selected for GIFs by using over 100K user generated GIFs and their corresponding video sources. We effectively deal with the noisy web data by proposing a novel adaptive Huber loss in the ranking formulation. We show that our approach is robust to outliers and picks up several patterns that are frequently present in popular animated GIFs. On our new large-scale benchmark dataset, we show the advantage of our approach over several state-of-the-art methods.

==> method_backup.tex <==

%-----------------------------------------
% Method
%-----------------------------------------
\section{Method}
Our goal is to detect segments of a video suitable as animated GIFs. We start by segmenting a video into a set of non-overlapping segments $\mathcal{S}$, using the video shot segmentation algorithm of~\cite{Song}. This algorithm creates segments by finding multiple change-points in a multi-dimensional sequence, which are considered to be segment boundaries.
%We target the task of automatically finding video segments suitable as GIFs.
%A good GIF is a short snippet of  special moments, facial expressions or funny events.

In testing, we compute the highlight score $h(s)$ of a segment $s \in \mathcal{S}$, where we learn the mapping function $h(\cdot)$ using a neural network. Higher scores indicate that a segment makes a better GIF.

\subsection{Training objective}
\label{sec:objective}
%In order to learn the mapping $h(s)$, we rely on the training data obtained in the previous section.
%The data corresponds to a set of segments, labeled with whether they are part of a GIF of not.
%The goal of training is thus to learn a mapping that allows to find segments that are suitable as GIFs.
A straightforward approach to formulate our problem is posing it as a classification task, where segments selected for GIFs are considered positive and others as negative. In testing, the posterior probability of the classification result on a segment can be used to obtain its ranking. But given the subjectivity of the task, there exists no clear cut definition of what is a good or bad segments. Rather, there are various degrees of GIF suitability, where we can assume that a selected segment is more suitable than other non-selected segments. Thus, as confirmed in our experiments, the classification formulation of our problem is inadequate.

Instead, we can define a set of rank constraints over the dataset $\mathcal{D}$, where we require selected segments to rank higher than non-selected ones,~\ie
\begin{align*}
h(s^+) > h(s^-), \:\:\:\:
\forall s^+, s^- \in \mathcal{D}
\end{align*}
where the segments $s^+$ are part of a GIF, while $s^-$ are not.

Yet, it is not clear if a highlight from one video would be considered a highlight in another video. In some videos (\eg compilations and carefully edited videos), many segments are of interest, but some of them will be negatives, as not all can be selected for the GIF. In others, even the selected parts of the video are of low quality. The notion of a highlight in our training data is thus most meaningful only within and not across videos. To account for this, we relax the constraints to \Q{YS: You are actually constraining, instead of relaxing, the condition to be video specific.}
\begin{align*}
h(s^+) > h(s^-), \:\:\:\:
\forall s^+,s^- \in S.
\end{align*}
That is, we require a positive segment $s^+$ to score higher than negative segments $s^-$ that come from the same video only.

\bigskip
\noindent
\textbf{Loss function.}
As we have seen, the task is a ranking problem by nature. We therefore follow~\cite{Sun2014} and use a rank loss between pairs of segments from the same video. However, since our training data is crawled from online sources and, to some degree, subjective, the labels are expected to be noisy. Using an L2 loss which gives quadratic penalty to outliers as~\eg~\cite{Sun2014,Lee2014}, is thus inapt for the task at hand. Alternatively, one could simply use an L1 loss

\begin{equation}
l_1(\subsup{s}{}{+},\subsup{s}{}{-})=\max\left(0,1-h(s^+)+h(s^-)\right).
\end{equation}
\ie a positive segment is required to score higher than its negative counterpart by a margin of 1. If the margin is violated, the incurred loss is linear in the error. We however find that such a loss over-penalizes small margin violations. Thus, we propose a novel robust rank loss, which is an adaption of the Huber Loss~\cite{huber1964robust} to the ranking setting. The loss gives a low penalty to small violations of the margin (where the ranking is still correct) and is more robust to outliers, compared to the L2 loss. We define the loss as
\begin{equation}
\label{eq:loss}
%    l_{huber}(\subsup{s}{}{+},\subsup{s}{}{-}) = 
%\begin{cases}
%    0,                                   & \text{if }  h(s^+)-h(s^-)\geq 1\\
%   \frac{1}{2}\subsup{\left(h(\subsup{s}{}{-}) - h(\subsup{s}{}{+}) + 1 \right)}{}{2} , & \text{if } \delta \leq h(\subsup{s}{}{+})-h(\subsup{s}{}{-})\leq 1\\
%     \delta\(h(\subsup{s}{}{-}) -  h(\subsup{s}{}{+}) + 1\) -\frac{1}{2}\delta^2,                & \text{otherwise}
%\end{cases}
    l_{huber}(\subsup{s}{}{+},\subsup{s}{}{-}) = 
\begin{cases}
   \frac{1}{2}l_1^2, & \text{if } l_1 \leq \delta \\
     \delta l_1 -\frac{1}{2}\delta^2,                & \text{otherwise}
\end{cases}
\end{equation}
Thus, if the margin is violated, the loss corresponds to a Huber loss, which is squared for small margin-violations and linear for stronger violations. The parameter $\delta$ defines the point at which the loss becomes linear. We show the form of the three loss functions in Fig.~\ref{fig:loss}
%-----------------------------------------
\begin{figure}
\centering
\includegraphics[width=1.0\linewidth]{loss_functions.pdf}
\caption{\textbf{Rank loss comparison.} We show standard rank loss functions and our novel robust rank loss. The loss combines the robustness~\wrt to small margin violations of the L2 loss with the robustness to outliers of the L1 loss.}
\label{fig:loss}
\end{figure}
%-----------------------------------------

Finally, we define our objective function as the total loss over the dataset $\mathcal{D}$ with a squared L2 regularization on the model weights $\mathbf{w}$:
\begin{equation}
L(\mathcal{D},\mathbf{w}) = \sum_{S_i \in \mathcal{D}}\sum_{(s^+,s^-) \in S_i}  l_{huber}(\subsup{s}{}{+},\subsup{s}{}{-}) +\lambda||\mathbf{w}||^2_2,
\label{eq:loss_global}
\end{equation}
where $\lambda$ is the regularization parameter. \Q{YS: (1) It's actually a squared L2 norm; (2) the capital $\mathbf{W}$ usually refers to a matrix; I changed it to $\mathbf{w}$.}

%\begin{multline}
%\label{eq:loss}
%L(D,\mathbf{W}) = \sum_{S_i \in D}\sum_{(s^+,s^-) \in S_i} \max\left(0,1-h(s^+)+h(s^-)\right) \\ + \lambda||\mathbf{W}||^2_2,
%\end{multline}
%\ie a positive segment is required to score higher than its negative counterpart by a margin of 1.
%We compare global and video-specific labels in the experimental section.

\subsection{Network architecture}
Given that GIFs are chosen based on their semantic content and interesting motion, having a representation that captures these aspects is crucial. In order to capture the complex spatio-temporal dynamics of video segments, we use C3D as the segment representation, which has shown to be a strong generic feature for video classification~\cite{Tran2014a}. C3D adapts the architecture of AlexNet~\cite{Krizhevsky} to videos through a novel spatio-temporal convolution layer. In comparison to RGB-based features, they encode motion information while remaining computationally efficient.

We experimented with various network architectures. While the loss function turned out to be crucial, our experiments showed that the performance remains relatively stable for different network sizes. Thus, we opt for a simple 2 hidden layer full-connected model, where each hidden unit is followed by a ReLu non-linearity~\cite{nair2010rectified}. The final prediction layer, which outputs $h(s)$, is a simple single linear unit, predicting an unnormalized scalar score. As inputs to the network, we use segments represented with C3D features~\cite{Tran2014a}. We use \ATT{1024} units in the first and \ATT{256} in the second hidden layer. The final network has 4.457.985 parameters. The structure of our model is depicted in Fig.~\ref{fig:architecture}.

In order to decrease the variance of our model, we use a simple form of model averaging, where we use different snapshots of the learned model and average their predicted scores.

\begin{figure}
\centering
\includegraphics[clip,trim=0 0 0 0, width=1.0\linewidth]{architecture.pdf}
\caption{The architecture of our proposed network. Trainable layers are shown in {\color{green}green}. Each hidden layer is followed by a ReLu non-linearity~\cite{nair2010rectified}. The final scoring layer is a linear function of the last hidden layer. The rank loss acts on pairs of segments and is non-zero, unless $s^+$ scores higher than $s^-$ by a margin of 1. To emphasize that the loss acts on pairs of segments, we show the two passes separately, but we use a single network.}.
\label{fig:architecture}
\end{figure} 
 
\subsection{Optimization}
In order to minimize the loss defined in Eq.~\ref{eq:loss_global}, we use backpropagation~\cite{rumelhart1985learning} with minibatch stochastic gradient descent. We use mini-batches of 50 pairs. In order to accelerate convergence, we apply Nesterov's Accelerated Momentum~\cite{bengio2013advances} for updating the weights. Momentum is set to 0.9 and $\lambda=0.001$ (weight decay). We initialize training with a learning rate of \ATT{$0.001$} and reduce it every 10th epoch. The learning is stopped after \ATT{25} epochs. Since our training data is obtained by leveraging web sources, the labels are noisy. Regularizing the network to avoid fitting the noise is thus of crucial importance. We applied dropout~\cite{Hinton2014} regularization to all hidden layers (\ATT{0.8 for the input layer and 0.2 for the first hidden layer}, respectively). Dropout is a simple, approximate way to do model averaging which increases robustness of the model~\cite{Hinton2014}.

The models were implemented using Theano~\cite{bergstra2010theano} with Lasagne~\cite{sander_dieleman_2015_27878}.


==> notes.tex <==

\section{Notes/TODOs}
Claims:
(i) Autogif is novel 
(ii) Rank better than classification 
(iii) Rank within video is meaningful, across videos is not --> Train with same number of pairs
(iv) Dataset results: AlexNet classes.
(v) Experiments: The way we do context doesn't help the way we do it. Encoded in the segment features? RNNs could help?


CC GIFs as examples:
sN9yXL (donkeys),RgdbIn (tire) ,8fSJ3C (bike theft),O9RvHN (negative example), 2uScbU (cats) ,gO468K (dog on stairs), LShYQX (happy dog), PibfsJ (sleep running dog)

==> test_results.tex <==
\begin{table}
\centering
\begin{tabular}{|l|c|c|}
\hline
\textbf{Method} & \textbf{nMSD} & \textbf{mAP} \\
\hline
%Random scores & 52.64\% & 10.50\% \\
\hline
Joint embedding~\cite{Liu2015} & 54.38\%  & 9.65\% \\
Category-spec. SVM~\cite{Potapov2014} & 54.43\%  & 9.88\% \\
Domain-spec. rankSVM~\cite{Sun2014} & 46.40\%  & 14.05\%  \\
\hline
\hline
Classification &  61.37\% & 8.81\% \\
Rank, video agnostic & 53.16\% & 11.37\% \\
\hline
Rank, $l_1$ loss & 45.50\% & 13.93\%	 \\
Rank, $l_2$ loss & 44.43\% & 14.12\% \\
\hline
Rank, Huber loss & 44.46\% & \textbf{14.54\%} \\
Rank, adaptive Huber loss & 44.53\% & 14.32\% \\
\hline
\hline
 \parbox{5cm}{Rank, adaptive Huber loss \\ + context (Ours)} & 43.94\%  & 14.45\% \\
\hline
Ours + model averaging & \textbf{43.74\%} & 14.29\% \\
\hline
\hline
Approx. bounds & 38.08\%  & 22.52\% \\
\hline
\end{tabular}
\caption{Experimental results. A lower nMSD and higher mAP represent better performance.  }
%Interestingly, our method shows no significant increase in performance when including metadata. This suggests that this information is already contained in the C3D segment representation.
\label{tab:test_results}
\end{table}


==> test_results_extended.tex <==
\begin{table}
\centering
{\small
\begin{tabular}{|l|l|l|}
\hline
\textbf{Method} & \textbf{mAP} & \textbf{MSD} \\
%\hline
%Random scores (100 runs) & 14.42\%  & 52.77\% \\
\hline
\hline
Domain-spec. rankSVM~\cite{Sun2014} & 17,64\% (+3,2) & 47,42\% (-5,3) \\
Joint embedding~\cite{Liu2015} & 14,83\% & 51,78\% \\
Category-spec. SVM~\cite{Potapov2014} & 13.63\% & 55.40\% \\
\hline
\hline
Classification & 15.12\% & 52.96\% \\
Rank, video agnostic & 15.27 \% & 52.32\%\\
\hline
Rank, $l_1$ loss & 17.52\% & 46.00\% \\
Rank, $l_2$ loss & 17.19\% & 47.61\% \\
\hline
Rank, Huber loss & 18.09\% & 45.07\% \\
Rank, adaptive Huber loss & & \\
\hline
Rank, adaptive Huber & & \\ + context (Ours)
 & & \\
\hline
Ours + model averaging & 18.54\% (+4.1) & 45.61\% (-7.2) \\
\hline
\hline
Approx. upper bound & 24.68\%  (+10.2) & 38.29\% (-13.5) \\
\hline
\end{tabular}
}
\caption{Results on the test set. Our method outperforms previous methods. 
In particular using our robust Huber rank loss leads to a significant performance increase over traditional losses.
For MSD, lower is better.}
\label{tab:test_results}
\end{table}


==> validation_results.tex <==
\begin{table}
\centering
\begin{tabular}{|l|c|}
\hline
Random (2015-09-21) & 0.0891 \\
Early frames (2015-09-21) & 0.1219 \\
\hline
Domain Specific rankSVM (2015-09-23) & 0.1078 \\
\hline
RankNet (2015-09-21) & 0.1499 \\
RankNet crossvideo labels (2015-09-24) & 0.1257 \\
\hline
\end{tabular}
\caption{Results on the validation set}
\label{tab:val_results}
\end{table}

